Updating Embeddings for Dynamic Knowledge Graphs

Data in Knowledge Graphs often represents part of the current state of the real world. Thus, to stay up-to-date the graph data needs to be updated frequently. To utilize information from Knowledge Graphs, many state-of-the-art machine learning approaches use embedding techniques. These techniques typically compute an embedding, i.e., vector representations of the nodes as input for the main machine learning algorithm. If a graph update occurs later on -- specifically when nodes are added or removed -- the training has to be done all over again. This is undesirable, because of the time it takes and also because downstream models which were trained with these embeddings have to be retrained if they change significantly. In this paper, we investigate embedding updates that do not require full retraining and evaluate them in combination with various embedding models on real dynamic Knowledge Graphs covering multiple use cases. We study approaches that place newly appearing nodes optimally according to local information, but notice that this does not work well. However, we find that if we continue the training of the old embedding, interleaved with epochs during which we only optimize for the added and removed parts, we obtain good results in terms of typical metrics used in link prediction. This performance is obtained much faster than with a complete retraining and hence makes it possible to maintain embeddings for dynamic Knowledge Graphs.

==> fragments.tex <==

\todo[inline]{MC It is unclear whether these parts have been rewritten or not!!!!!!!!!!}

\section{Knowledge Graph Embedding}


Nowadays, there is a large variety of different embedding models for knowledge graphs, which have been summarized by Wang et al. ~\cite{Survey}.
While translational distance models like \textsc{TransE}~\cite{TransE} and semantic matching models like \textsc{DistMult}~\cite{DistMult} or \textsc{Rescal}~\cite{RESCALslides,RESCALpaper} leverage the information directly given by the facts (i.e. edges) of the KG, models like \textsc{RDF2Vec}~\cite{RDF2Vec} or \textsc{GloVe}~\cite{RDFGloVe} perform random walks to derive entity and relation sequences as input for neural language models like word2vec~\cite{word2vec}.
Although all of these three categories share the same task of computing an embedding as training data for machine learning models, \textsc{RDF2Vec} and \textsc{GloVe} embeddings are not supposed to be used for direct link prediction, i.e. without the training of a machine learning model for this certain task.
As the focus of this paper is on the embedding step itself, we limit ourselves to translational distance and semantic matching models in order to use direct link prediction for the measurement of embedding quality.
Since both of these categories are very similar, they can be generalized in the form of an abstract embedding model, which we are going to use in order to propose a general update step independent of the specific embedding method.

\subsection{An Abstract Embedding Model}
All embedding models have in common that the computation of the embedding is an incremental learning process.
To validate the improvement of the embedding in the training phase and to evaluate the resulting embedding, the triples $E$ from the KG $\mathcal{G}=(V, E)$ are separated into a training set $S$, a validation set $W$ and a test set $T$ with $S\mathbin{\dot{\cup}}W\mathbin{\dot{\cup}}T=E$.

Both, translational distance and semantic matching models, try to learn embeddings under the local closed world assumption~\cite{kv} (to apply negative sampling) by minimizing either the logistic loss
\begin{equation}\label{logistic_loss}
	\underset{\Theta}{\mathrm{min}}\sum_{(h,r,t)\in S\cup S'} \mathrm{log}(1+\mathrm{exp}(-y_{(h,r,t)}\cdot f_{r}(h,t)))
\end{equation}
or the pairwise ranking loss
\begin{equation}\label{pairwise_ranking_loss}
	\underset{\Theta}{\mathrm{min}}\sum_{(h,r,t)\in S}\sum_{(h',r,t')\in S'} [\gamma-f_{r}(h,t)+f_{r}(h',t')]_+
\end{equation}
where $\Theta$ is the current embedding of the KG, $S$ the training set, $S'=(V\times\mathcal{R}\times V) \setminus S$ the complement of the training set, $y_{(h,r,t)}=\pm 1$ a sign indicating, whether $(h,r,t)$ holds or not, 
$\gamma>0$ a margin hyperparameter, $[x]_+ = \mathrm{max}(0, x)$ and $f_{r}$ the model dependent scoring function for the relation $r$~\cite{Survey}.
The intuition behind the scoring functions $f_r:V\times V \rightarrow\mathbb{R}$ is to measure the plausibility of the relationship $r$ between a given head entity $h$ and a tail entity $t$.
Therefore, $f_r(h, t)$ is intended to have a higher score, if the triple $(h, r, t)$ is in the particular KG, than if it is not.
The loss function is minimized in the training phase using common stochastic gradient descent methods. 

\subsection{Dynamic Knowledge Graphs}
Before we propose a method to embed dynamic knowledge graphs, we need to formalize them as mathematical objects in order to introduce a consistent formalism.
To provide adaptability for as many use cases as possible, we keep the definitions general and also include a dynamic ontology (i.e. set of relations).
\begin{mydef}
	A dynamic knowledge graph $\mathcal{G}^{(t)}=(V^{(t)}, E^{(t)})$ at time step t over a dynamic set of relations $\mathcal{R}^{(t)}$ is defined as a pair of:
	\begin{itemize}
		\item vertices $V^{(t)}$ at time step t and
		\item edges $E^{(t)}\subseteq V^{(t)}\times \mathcal{R}^{(t)} \times V^{(t)}$ at time step t.
	\end{itemize}
\end{mydef}
To formalize the dynamics of an evolving KG, we consider the differences of the graph at two consecutive time steps by introducing the definition of change.
\begin{mydef}\label{definition_change}
	The change of the dynamic knowledge graph $\mathcal{G}^{(t+1)}=(V^{(t+1)}, E^{(t+1)})$ over the set of relations $\mathcal{R}^{(t+1)}$ at time step t+1 compared to $\mathcal{G}^{(t)}=(V^{(t)}, E^{(t)})$ over $\mathcal{R}^{(t)}$ at time step t is defined by:
	\begin{itemize}
		\item the additions $\Delta V^{+}=V^{(t+1)}\setminus V^{(t)}$ and deletions $\Delta V^{-}=V^{(t)}\setminus V^{(t+1)}$ of vertices,
		\item the additions $\Delta E^{+}=E^{(t+1)}\setminus E^{(t)}$ and deletions $\Delta E^{-}=E^{(t)}\setminus E^{(t+1)}$ of edges and
		\item the additions $\Delta \mathcal{R}^{+}=\mathcal{R}^{(t+1)}\setminus\mathcal{R}^{(t)}$ and deletions $\Delta \mathcal{R}^{-}=\mathcal{R}^{(t)}\setminus\mathcal{R}^{(t+1)}$ of relations.
	\end{itemize}
\end{mydef}

\subsection{Evaluation of Dynamic Graph Embeddings}
The goal of this paper is to allow the embedding of a dynamic KG to be trained simultaneously with machine learning models using it.
To achieve this goal, we formulate four main properties, which we aim for in our approach (referred to as updates):
\begin{enumerate}\label{properties}
	\item \textbf{High-quality Approximation} - The updates are required to be a good approximation of complete recalculations to keep the quality of the embedding predictable.
	\item \textbf{Stability} - As we assume that a stable embedding is better suited for continuing the training of machine learning models, the embedding of a dynamic KG should evolve smoothly to provide this stability.
	\item \textbf{Low Time Complexity} - The updates should be faster than recalculating the whole embedding to allow continuous adjustments, while the KG is evolving.
	\item \textbf{Scalability} - The online model should be able to scale up to today's large-scale KGs.
\end{enumerate}
To measure the quality of embeddings, we use link prediction as the standard evaluation task for embedding models in previous work~\cite{Survey}. For this, we employ the two widely used metrics Mean Rank and Hits@10.

\subsubsection{Stability Measure}
We call an embedding stable, if its vectors do not change significantly during training.
Therefore, the stability should describe the degree of discrepancy between two consecutive embeddings of a dynamic KG.
To our knowledge, there are no techniques to measure this notion of embedding stability so far.
Therefore, we define the Normalized Mean Change (NMC) for the entity representations (analogously for relations) of two consecutive embeddings $\Theta^{(t)}$ and $\Theta^{(t+1)}$ of a dynamic KG $\mathcal{G}$ as
\begin{equation}\label{NMC}
	NMC=\frac{1}{dist_\varnothing}\sum_{v\in V_{sh}}\frac{\mathrm{dist}(\vec{v}^{(t+1)}, \vec{v}^{(t)})}{\sum_{w\in V_{sh}}\mathrm{dist}(\vec{v}^{(t+1)}, \vec{w}^{(t+1)})}
\end{equation}
where $V_{sh}=V^{(t+1)}\cap V^{(t)}$ is the set of shared entities at both time steps, $\vec{v}^{(t)}$ the embedding of entity $v$ at time step $t$ and \[dist_\varnothing=\frac{1}{|V_{sh}|}\sum_{(v, w)\in V_{sh}\times V_{sh}}\mathrm{dist}(\vec{v}^{(t+1)}, \vec{w}^{(t+1)})\] the average pairwise distance between shared entities with respect to the distance metric $\mathrm{dist}:\mathbb{R}^{d}\times \mathbb{R}^{d}\rightarrow\mathbb{R}$. 
The metric can be seen as the average distance between old and new vector representations with two normalization factors, because the semantics of the degree of distances depends on the overall distances in the embedding.
First, we normalize the distances for each entity individually using the average distance to all other entities at time step $t+1$ to consider local clusters.
Secondly, to allow comparability of different embeddings globally, we normalize it again by $dist_\varnothing$.
Note that the normalization factors $\frac{1}{|V_{sh}|}$ of the average in the denominator of each summand and of the outer average over $v\in V_{sh}$ cancel each other out.
For the distance metric, we employ the $L_1$-, $L_2$- and cosine-distances.

\subsubsection{Dynamic Training, Validation and Test Sets}
To combine the usually static training, validation and test sets with the dynamics of an evolving KG, we introduce a dynamic training set $S^{(t)}$, a dynamic validation set $W^{(t)}$ and a dynamic test set $T^{(t)}$ with $S^{(t)}\mathbin{\dot{\cup}}W^{(t)}\mathbin{\dot{\cup}}T^{(t)}=E^{(t)}$.
In order to 

